Deep Visual Odometry with Adaptive Memory

We propose a novel deep visual odometry (VO) method that considers global information by selecting memory and refining poses. Existing learning-based methods take the VO task as a pure tracking problem via recovering camera poses from image snippets, leading to severe error accumulation. Global information is crucial for alleviating accumulated errors. However, it is challenging to effectively preserve such information for end-to-end systems. To deal with this challenge, we design an adaptive memory module, which progressively and adaptively saves the information from local to global in a neural analogue of memory, enabling our system to process long-term dependency. Benefiting from global information in the memory, previous results are further refined by an additional refining module. With the guidance of previous outputs, we adopt a spatial-temporal attention to select features for each view based on the co-visibility in feature domain. Specifically, our architecture consisting of Tracking, Remembering and Refining modules works beyond tracking. Experiments on the KITTI and TUM-RGBD datasets demonstrate that our approach outperforms state-of-the-art methods by large margins and produces competitive results against classic approaches in regular scenes. Moreover, our model achieves outstanding performance in challenging scenarios such as texture-less regions and abrupt motions, where classic algorithms tend to fail.

==> Sections/Introduction20181112.tex <==
\IEEEraisesectionheading{\section{Introduction}}
\IEEEPARstart{V}{isual} Odometry (VO) and Visual Simultaneous Localization And Mapping (V-SLAM) estimate camera poses from image sequences by exploiting the consistency between consecutive frames. 
As an essential task in autonomous driving and robotics, VO has been studied for decades and many outstanding algorithms have been developed \cite{mur2017orb-slam2, engel2014lsd-slam, engel2018dso, wang2017stereo, geiger2011stereoscan}. Recently, as Convolutional Neural Networks (CNNs) and Recurrent Neural Networks (RNNs) achieve impressive performance in many computer vision tasks \cite{yang2018dvso, dosovitskiy2015flownet, brahmbhatt2018mapnet, henriques2018mapnet}, a number of end-to-end models have been proposed for VO estimation. These methods either learn depth and ego-motion jointly with CNNs \cite{zhou2017egomotion, zhan2018feature, yin2018geonet, li2018undeepvo, mahjourian2018vid2depth}, or leverage RNNs to introduce temporal information \cite{wang2017deepvo, wang2018espvo, xue2018fea, parisotto2018gpe, iyer2018ctc}. Due to the high dimensionality of depth maps, the number of frames is commonly limited to no more than 5. Although temporal information is aggregated through recurrent units, RNNs are incapable of remembering previous observations for long time \cite{sukhbaatar2015memory}, leading to the limited usage of historical information. Besides, the above methods pay little attention to the significance of incoming observations for refining previous results, which is crucial for VO tasks. 

\input{fig_table/table_methods}

\begin{figure}[t]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1.\linewidth]{images/overview5S}
	\end{center}
	\label{fig:framework}
	\caption{Overview of our framework. Compared with existing learning-based methods which formulate VO task as a pure tracking problem, we introduce two useful components called \textit{Memory} and \textit{Refining}. The \textit{Memory} module preserves longer time information by adopting an adaptive context selection strategy. The \textit{Refining} module ameliorates previous outputs by employing a spatial-temporal feature reorganization mechanism.}
\end{figure}

Direct estimation of camera motions from image snippets is prone to large errors due to the geometric uncertainty caused by \textit{small baselines} (especially for handheld devices). Consequently, error accumulation is getting increasingly severe over time, as global poses are integrated from frame-wise poses. In classic VO/SLAM systems \cite{mur2017orb-slam2}, a local map is established according to the co-visibility graph over up to hundreds of frames, on which bundle adjustment is executed to jointly optimize all corresponding poses. Therefore, both previous and new observations are incorporated for optimization, and accumulated errors are thus alleviated. 

Inspired by classic VO/SLAM systems \cite{mur2017orb-slam2, engel2018dso}, we introduce an effective component, called \textit{Memory}, which explicitly preserves the accumulated information adaptively. Owing to the high sample frequency, contents between consecutive frames are much overlapped. Rather than keeping accumulated information per time step with brute force, an intuitive and efficient strategy is utilized to reduce the redundancy.
% \cite{engel2013svo}
As errors of previous poses will propagate over time to current estimation, refining previous results becomes necessary. The \textit{Memory} contains more \textit{global} information, which can be leveraged naturally to refine previous results. Therefore, a \textit{Refining} component is introduced. The \textit{Refining} module takes the global pose estimation as a registration problem by aligning each view with the \textit{Memory}.
A spatial-temporal attention mechanism is applied to the contexts stored in the \textit{Memory} for feature selection.

The overview of our framework is illustrated in Fig.~\ref{fig:framework}. The encoder encodes paired images into high-level features. The \textit{Tracking} module accepts sequential features as input, fuses current observation into accumulated information using convolution LSTMs \cite{xingjian2015convolutional} for preserving spatial connections, and produces relative poses. Hidden states of the \textit{Tracking} RNN are adaptively preserved in the \textit{Memory} slots. The \textit{Refining} module ameliorates previous results using another convolutional LSTM, enabling refined results passing through recurrent units to improve the following outputs. Our contributions can be summarized as follows:
% The entire framework can be trained in an end-to-end fashion.
\begin{itemize}
	%\item We propose a novel end-to-end deep VO framework extending the field of view by preserving memories selectively, and thus reducing the geometric uncertainty;
	%\item We employ a two-stage learning strategy for tracking and refinement, hence previous results can be refined and further improve the performance of whole system in dealing with error accumulation;
	\item We propose a novel end-to-end VO framework consisting of the \textit{Tracking}, \textit{Memory} and \textit{Refining} components;
	\item An adaptive and efficient strategy is adopted for the \textit{Memory} component to preserve accumulated information;
	%\item The \textit{Memory} module preserves the accumulated information by adopting an adaptive and efficient strategy;
	\item A spatial-temporal attention mechanism is employed for the \textit{Refining} component to distill valuable features.
	%\item The \textit{Refining} module distills valuable features by employing a spatial-temporal attention mechanism.
	%\item Our method outperforms state-of-the-art learning-based VO methods and it gives competitive results against classic VO algorithms. Additionally, it works well in challenging conditions where classic algorithms tend to fail due to insufficient textures or abrupt motions.
\end{itemize}

Our method outperforms state-of-the-art learning-based methods and produces competitive results against classic algorithms. Additionally, it works well in challenging conditions where classic algorithms tend to fail due to insufficient textures or abrupt motions. The rest of this paper is organized as follows. In Sec.~\ref{related_work}, related works on monocular odometry are discussed. In Sec.~\ref{method}, our architecture is described in detail. The performance of the proposed approach is compared with current state-of-the-art methods in Sec.~\ref{experiment}. We conclude the paper in Sec.~\ref{conclusion}.  

==> fig_table/table_tum_frames.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{3.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{ccc||cccccc}
				\hline
				\hline
				Sequence & \makecell{Desc. \\ str/tex/abrupt motion}& Frames & \makecell{5 frames}  & \makecell{ 7 frames} & \makecell{9 frames} & \makecell{11 frames}\\
				\hline
				fr2/desk & Y/Y/N & 2965  & 0.183  & 0.164 & 0.159 & 0.153 \\
				%fr2/360\_hemisphere & Y/Y/N & X & X  & 0.158  & 0.154 & 0.170 & 0.231 \\
				fr2/360\_kidnap & Y/Y/N & 1431  & 0.313  & 0.225 & 0.224 & 0.208 \\
				fr2/pioneer\_360  & Y/Y/Y & 1225 & 0.241  & 0.1338 & 0.076 & \textbf{0.056} \\
				fr2/pioneer\_slam3 & Y/Y/Y & 2544 & 0.149  & 0.1065 & 0.085 & \textbf{0.070}\\
				%fr2/dishes & Y/Y/N & \textbf{0.070} & 0.133  & 0.1448  & 0.1210 & 0.088 & 0.081 \\
				fr2/large\_cabinet & Y/N/N & 1011 & 0.193  & 0.193 & 0.177 & \textbf{0.172} \\
				fr3/sitting\_static & Y/Y/N & 707 & 0.017  & 0.018 & 0.017 &\textbf{0.015} \\
				%fr3/sitting\_xyz & 0.021 & 0.044  & 0 & 0 & 0 & 0.201 & object\\
				%fr3/cabinet & Y/N/N & X & 2.531  & 0.1578   & 0.1660 & 0.190 & 0.196 \\
				fr3/nstr\_ntex\_near\_loop & N/N/N & 1125 & 0.371 & 0.195 & 0.157 & \textbf{0.123} \\ 
				fr3/nstr\_tex\_near\_loop & N/Y/N & 1682   & 0.046  & 0.011 & 0.010 & \textbf{0.007} \\ 
				fr3/str\_ntex\_far & Y/N/N & 814 & 0.069  & 0.047 & 0.039 & \textbf{0.035} \\ 
				fr3/str\_tex\_far & Y/Y/N & 938 & 0.080  & 0.049 & 0.046 &0.042 \\ 
				\hline
				\hline
			\end{tabular}	
		\end{center}
	\caption{Evaluation on the TUM-RGBD dataset \cite{tum12iros}. The values describe the translational RMSE in [m/s]. Results of our model with the \textit{Tracking}, \textit{Memory} and \textit{Refining} components on sequence lengths of 5, 7, 9,11.}
	\label{table:tum}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{2cm}
